Beyond Deep Ensembles: A Large-Scale Evaluation of Bayesian Deep Learning under Distribution Shift

Bayesian deep learning (BDL) is a promising approach to achieve well-calibrated predictions on distribution-shifted data. Nevertheless, there exists no large-scale survey that evaluates recent SOTA methods on diverse, realistic, and challenging benchmark tasks in a systematic manner. To provide a clear picture of the current state of BDL research, we evaluate modern BDL algorithms on real-world datasets from the WILDS collection containing challenging classification and regression tasks, with a focus on generalization capability and calibration under distribution shift. We compare the algorithms on a wide range of large, convolutional and transformer-based neural network architectures. In particular, we investigate a signed version of the expected calibration error that reveals whether the methods are over- or under-confident, providing further insight into the behavior of the methods. Further, we provide the first systematic evaluation of BDL for fine-tuning large pre-trained models, where training from scratch is prohibitively expensive. Finally, given the recent success of Deep Ensembles, we extend popular single-mode posterior approximations to multiple modes by the use of ensembles. While we find that ensembling single-mode approximations generally improves the generalization capability and calibration of the models by a significant margin, we also identify a failure mode of ensembles when finetuning large transformer-based language models. In this setting, variational inference based approaches such as last-layer Bayes By Backprop outperform other methods in terms of accuracy by a large margin, while modern approximate inference algorithms such as SWAG achieve the best calibration.

==> posterior_approx.tex <==
\section{Quality of Posterior Approximations}
\label{sec:hmc-compare}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \begin{tikzpicture}
            \def\bayesdatafile{data/cifar10.dat}
            \def\bayesxcol{corruption}
            \def\bayesfiltercol{model}
            \def\bayesycol{sece}
            \def\bayesyerr{sece_std}

            \begin{axis}[
                    paretostyle,
                    width=\textwidth,
                    height=3cm,
                    every axis plot/.append style={
                        draw=none
                    },
                    xlabel={\tiny sECE},
                    ylabel={\tiny Corruption},
                    ytick=data,
                    yticklabels = {0, 1, 3, 5},
                    y dir=reverse,
                    xmin=-0.29,
                    xmax=0.13,
                    xticklabel style={
                        /pgf/number format/fixed,
                        /pgf/number format/precision=2
                    }
                ]
                \draw[dashed] (axis cs:0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs:0,\pgfkeysvalueof{/pgfplots/ymax}); %
                \modelplot{hmc}{HMC}{color=hmc, single, mark size=2pt}
                \modelplot{MAP}{MAP}{color=map, single, mark size=2pt}
                \modelplot{Deep Ensemble}{Deep Ensemble}{color=map, multix, mark size=2pt}
                \modelplot{MCD}{MCD}{color=mcd, single, mark size=2pt}
                \modelplot{MultiMCD}{MultiMCD}{color=mcd, multix, mark size=2pt}
                \modelplot{SWAG}{SWAG}{color=swag, single, mark size=2pt}
                \modelplot{MultiSWAG}{MultiSWAG}{color=swag, multix, mark size=2pt}
                \modelplot{BBB}{BBB}{color=bbb, single, mark size=2pt}
                \modelplot{bbb_5}{MultiBBB}{color=bbb, multix, mark size=2pt}
                \modelplot{Rank1}{Rank1}{color=rank1, single, mark size=2pt}
                \modelplot{iVON}{iVON}{color=ivon, single, mark size=2pt}
                \modelplot{ivon_5}{MultiiVON}{color=ivon, multix, mark size=2pt}
                \modelplot{Laplace}{Laplace}{color=laplace, single, mark size=2pt}
                \modelplot{laplace_5}{MultiLaplace}{color=laplace, multix, mark size=2pt}
                \modelplot{SVGD}{SVGD}{color=svgd, single, mark size=2pt}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
        \centering
        \begin{tikzpicture}
            \def\bayesdatafile{data/cifar10.dat}
            \def\bayesxcol{corruption}
            \def\bayesfiltercol{model}
            \def\bayesycol{tv}
            \def\bayesyerr{tv_std}

            \begin{axis}[
                    paretostyle,
                    width=\textwidth,
                    height=3cm,
                    every axis plot/.append style={
                        draw=none
                    },
                    xlabel={\tiny Total Variation},
                    ylabel={\tiny Corruption},
                    ytick=data,
                    yticklabels = {0, 1, 3, 5}, %
                    y dir=reverse,
                    xmin=0.102,
                    xmax=0.398
                ]

                \modelplot{MAP}{MAP}{color=map, single, mark size=2pt}
                \modelplot{MCD}{MCD}{color=mcd, single, mark size=2pt}
                \modelplot{MultiMCD}{MultiMCD}{color=mcd, multix, mark size=2pt}
                \modelplot{SWAG}{SWAG}{color=swag, single, mark size=2pt}
                \modelplot{MultiSWAG}{MultiSWAG}{color=swag, multix, mark size=2pt}
                \modelplot{BBB}{BBB}{color=bbb, single, mark size=2pt}
                \modelplot{bbb_5}{MultiBBB}{color=bbb, multix, mark size=2pt}
                \modelplot{Rank1}{Rank1}{color=rank1, single, mark size=2pt}
                \modelplot{iVON}{iVON}{color=ivon, single, mark size=2pt}
                \modelplot{ivon_5}{MultiiVON}{color=ivon, multix, mark size=2pt}
                \modelplot{Laplace}{Laplace}{color=laplace, single, mark size=2pt}
                \modelplot{laplace_5}{MultiLaplace}{color=laplace, multix, mark size=2pt}
                \modelplot{SVGD}{SVGD}{color=svgd, single, mark size=2pt}
                \modelplot{Deep Ensemble}{Deep Ensemble}{color=map, multix, mark size=2pt}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
        \centering
        \resizebox{.7\textwidth}{!}{
            \begin{tikzpicture}
                \begin{axis}[
                        paretostyle,
                        xmin=0, xmax=1, ymin=0, ymax=1,
                        hide axis,
                        legend columns=8,
                        legend style={
                            legend cell align=left
                        }
                    ]
                    
                    \addlegendimage{color=map, single}
                    \addlegendentry{MAP};
                    \addlegendimage{color=mcd, single}
                    \addlegendentry{MCD};
                    \addlegendimage{color=swag, single}
                    \addlegendentry{SWAG};
                    \addlegendimage{color=bbb, single}
                    \addlegendentry{BBB};
                    \addlegendimage{color=laplace, single}
                    \addlegendentry{Laplace};
                    \addlegendimage{color=ivon, single}
                    \addlegendentry{iVON};
                    \addlegendimage{color=rank1, single}
                    \addlegendentry{Rank-1 VI};
                    \addlegendimage{color=hmc, single}
                    \addlegendentry{HMC};

                    
                    \addlegendimage{color=map, multix}
                    \addlegendentry{Deep Ensemble};
                    \addlegendimage{color=mcd, multix}
                    \addlegendentry{MultiMCD};
                    \addlegendimage{color=swag, multix}
                    \addlegendentry{MultiSWAG};
                    \addlegendimage{color=bbb, multix}
                    \addlegendentry{MultiBBB};
                    \addlegendimage{color=laplace, multix}
                    \addlegendentry{MultiLaplace};
                    \addlegendimage{color=ivon, multix}
                    \addlegendentry{MultiiVON};
                    \addlegendimage{color=svgd, single}
                    \addlegendentry{SVGD};
                \end{axis}
            \end{tikzpicture}
        }
    \end{subfigure}

                    
        
        
    

    \caption{\dataset{CIFAR-10-(C)}: sECE (closer to zero is better) and total variation (TV, smaller is better) between the model's predictions and HMC's predictions on the evaluation split of \dataset{CIFAR-10} (corruption $0$) and under increasing levels of image corruption by noise, blur and weather and digital artifacts (corruption $1, 3, 5$). Most single-mode approximations are overconfident, as indicated by the negative sECE. Ensembling makes the models less confident, with MultiSWAG and MultiiVON becoming underconfident, as indicated by the positive sECE. Considering the TV, MultiX consistently approximates the posterior better than the corresponding single-mode approximations, with MultiiVON and MultiSWAG achieving the smallest TV. The single-mode approximations SWAG, MCD and iVON approximate the posterior better than the Deep Ensemble.}
    \label{fig:cifar-all}
\end{figure}

While approximate inference is commonplace in Bayesian deep learning, the large size of the neural networks and datasets typically makes it computationally intractable to measure how well a model approximates the true parameter posterior.
Following \citet{wilson2021competition}, we measure the approximation quality of a model by the total variation (TV) between the model's predictions and HMC and the top-1 agreement with HMC.
To this end, we use the high-quality Hamiltonian Monte Carlo (HMC) \citep{neal1996bayes-nn} samples provided by \citet{izmailov2021bma-analysis} for CIFAR-10 \citep{krizhevsky09cifar}.
We compare the considered algorithms (see \Cref{sec:algos}) on the standard evaluation split of \dataset{CIFAR-10} as well as the corruption levels $1$, $3$, and $5$ of \dataset{CIFAR-10-C} \citep{hendrycks2019cifar-c}, where images are corrupted with increasing levels of noise, blur, and weather and digital artifacts.
\Cref{fig:cifar-all} displays the sECE and the TV of the evaluated models under varying levels of image corruption.
For further results regarding the accuracy, ECE, and top-1 agreement with HMC see \Cref{sec:cifar-details}.



\paragraph{Posterior Approximation Quality}
Overall, a good probabilistic single-mode approximation is the most important factor.
MultiX consistently approximates the posterior better 
Overall, MultiiVON approximates the posterior best across all corruption levels as measured by the TV, with MultiSWAG being a close contender.
MultiX models consistently approximate the parameter posterior better than single-mode approximations and the Deep Ensemble.
Even single-mode approximations such as MCD and SWAG achieve better TVs under data corruption than the Deep Ensemble.
As expected, MAP has the highest TV, with only a small improvement made by Laplace.

\paragraph{Calibration}
Most models become more overconfident under increasing levels of image corruption.
MCD and particularly SWAG are overall well calibrated, while BBB is more overconfident than MAP.
BBB's overconfidence is not an issue of the mean field approximation: iVON is comparatively well calibrated while using the same posterior approximation as BBB.
Rank-1 VI is comparatively well calibrated, likely due to its multi-modal posterior which gives it ensemble-like properties.
The Laplace approximation is only marginally better calibrated than MAP.
MultiX is generally underconfident, with MultiSWAG staying underconfident even under heavy image corruption.
This is in line with the overall underconfidence of HMC.
However, even HMC becomes overconfident on the highest corruption level, indicating that even the true Bayesian posterior is not perfectly calibrated.


==> scaling.tex <==
\section{Experiments under Realistic Distribution Shift}
\label{sec:scaling}
We now present a large-scale comparison of the BDL algorithms introduced in \Cref{sec:algos}.
We are interested in i) the ability of the models to generalize to distribution-shifted data, as measured by task-specific accuracy metrics that are based on real-world applications, and ii) the calibration of the models under distribution shift.
To this end we are using a subset of the WILDS dataset collection \citep{koh2021wilds}.
WILDS consists of ten diverse datasets that originate from real-world applications of deep learning in which models need to perform well under distribution shift.
Compared to standard o.o.d. datasets such as \dataset{MNIST-C} \citep{mu2019mnistc}, \dataset{CIFAR-10-C} \citep{hendrycks2019cifar-c} and UCI-Gap \citep{foong2019gap}, WILDS represents real-world distribution shift and is therefore more suitable for an application-oriented evaluation of BDL.
We systematically evaluate all algorithms on six of the ten datasets: The image-based regression task \dataset{PovertyMap} (\Cref{sec:image-regression}), the image classification tasks \dataset{iWildCam}, \dataset{FMoW}, and \dataset{RxRx1} (\Cref{sec:image-classification}), and the text classification datasets \dataset{CivilComments} and \dataset{Amazon} (\Cref{sec:text-classification}).
Aside from \dataset{PovertyMap}, all datasets are finetuning tasks, where we initialize the model's parameters from a model that has been pretrained on a similar task.
We also evaluated most algorithms on the \dataset{Camelyon17} image classification dataset but found that the performance degradation on the o.o.d. evaluation split was to a large part a consequence of the use of batch normalization rather than the o.o.d. data, making the datasets less interesting for a fair comparison on o.o.d. data (see \Cref{sec:batchnorm} for details).
We report results for the smaller UCI \citep{dua2017uci} and UCI-Gap \citep{foong2019gap} tabular regression datasets in \Cref{app:uci}.

As we want to evaluate the posterior approximation, generalization, and calibration capability of all models given the true parameter posterior, none of our models uses the metadata (e.g. location, time) associated with the input data, nor do we consider approaches that are specifically designed for o.o.d generalization or augment the dataset, for example by re-weighting underrepresented classes, contrary to the algorithms evaluated by \citet{koh2021wilds}.
We report all results with a $95\%$ confidence interval.


\subsection{Large-Scale Regression}
\label{sec:image-regression}

\paragraph{Task}
\dataset{PovertyMap-wilds} \citep{yeh2020povertymap} is an image-based regression task, where the goal is to better target humanitarian aid in Africa by estimating the asset wealth index of an area using satellite images.
As this task is significantly easier when buildings are visible in the images, the evaluation set is split into images containing urban and images containing rural areas.
The accuracy of the models is evaluated on both splits by the Pearson coefficient between their predictions and the ground truth asset wealth index, and the worst Pearson coefficient is used as the main evaluation metric.
See \Cref{sec:poverty-details} for details.


\begin{wrapfigure}[30]{r}{.5\textwidth}
    \centering
    \resizebox{.48\textwidth}{!}{
        \begin{tikzpicture}
            \def\bayesdatafile{data/poverty.dat}
            \def\bayesxcol{ood pearson}
            \def\bayesxerr{ood pearson_std}
            \def\bayesmodelcol{model}
            \begin{groupplot}[
                    paretostyle,
                    xlabel=Worst U/R Pearson,
                    height=7cm, width=7cm,
                    legend columns=1,
                    group style={
                        group size=3 by 1,
                        horizontal sep=2cm,
                        vertical sep=1.5cm
                    },
                ]
    
                \nextgroupplot[ylabel=sQCE, legend to name=povertylegend]
                    \plotcol{ood sqce}{ood sqce_std}
                    \modelparetoplot{map-1}{MAP}{color=map, single}
                    \addlegendentry{MAP};
                    \modelparetoplot{map-5}{Deep Ensemble}{color=map, multix}
                    \addlegendentry{Deep Ensemble};
                    \modelparetoplot{mcd-1}{MCD}{color=mcd, single}
                    \addlegendentry{MCD};
                    \modelparetoplot{mcd-5}{MultiMCD}{color=mcd, multix}
                    \addlegendentry{MultiMCD};
                    \modelparetoplot{swag-1}{SWAG}{color=swag, single}
                    \addlegendentry{SWAG}
                    \modelparetoplot{swag-5}{SWAG}{color=swag, multix}
                    \addlegendentry{MultiSWAG}
                    \modelparetoplot{bbb-1}{BBB}{color=bbb, single}
                    \addlegendentry{BBB};
                    \modelparetoplot{bbb-5}{MultiBBB}{color=bbb, multix}
                    \addlegendentry{MultiBBB};
                    \modelparetoplot{rank1-1}{Rank-1 VI}{color=rank1, single}
                    \addlegendentry{Rank-1 VI};
                    \modelparetoplot{laplace-1}{Laplace}{color=laplace, single}
                    \addlegendentry{Laplace};
                    \modelparetoplot{laplace-5}{MultiLaplace}{color=laplace, multix}
                    \addlegendentry{MultiLaplace};
                    \modelparetoplot{svgd-1}{SVGD}{color=svgd, single}
                    \addlegendentry{SVGD};
            \end{groupplot}
    
            \path (current bounding box.north east)--(current bounding box.south east) coordinate[midway] (group center);
            \node[xshift=2cm, yshift=0.5cm, inner sep=0pt] at(group center) {\pgfplotslegendfromname{povertylegend}};
        \end{tikzpicture}
    }

    \caption{\dataset{PovertyMap-wilds}: Worst urban/rural Pearson coefficient between the model's predictions and the ground-truth plotted against the sQCE on the o.o.d. test split of the image-based regression task.
    All models achieve similar, but noisy Pearson coefficients, indicating similar generalization capabilities.
    Multi-mode models are consistently better calibrated than single-mode models (note that Rank-1 VI's components and SVGD's particles give them multi-mode approximation capabilities).
    In regard to calibration, the relative ordering of the single-mode models does not translate to the MultiX models: BBB is among the best-calibrated single-mode models, but MultiBBB is the worst calibrated MultiX model.
    Laplace and SWAG are very similarly calibrated, therefore the data points of SWAG are hidden behind the data points of Laplace.
    iVON performs significantly worse than the other algorithms and is therefore excluded.}
    \label{fig:poverty-all}
\end{wrapfigure}
\paragraph{Generalization}
All models achieve similar Pearson coefficients, with MultiX, including the Deep Ensemble, being slightly more accurate. 
The Deep Ensemble is competitive with the best performing algorithm of the WILDS leaderboard \citep{wilds-leaderboard} with a Pearson coefficient of $0.52$ compared to $0.53$ of C-Mixup \citep{yao2022c-mixup}.
However, due to the large standard errors resulting from the different difficulties of the folds, the results are not significant.
Note that \citet{koh2021wilds} report similarly large standard errors.
iVON performs significantly worse than all other algorithms and is therefore excluded in \Cref{fig:poverty} (see \Cref{sec:poverty-details} for details).

\paragraph{Calibration}
The sQCE paints a clearer picture: While all models are overconfident, multi-mode posterior approximations are better calibrated than single-mode approximations.
MultiX, based on probabilistic single-mode approximations, is generally better calibrated than the Deep Ensemble.
SVGD is better calibrated than the Deep Ensemble, showing the benefit of the repulsive forces between the particles.


\subsection{Finetuning with Bayesian Principles}
Many Bayesian algorithms such as BBB and ensemble-based algorithms come with a significant increase in training time compared to MAP.
Combined with the ever-increasing size of modern deep neural networks, it becomes more and more expensive to apply Bayesian methods to state-of-the-art tasks.
However, fine-tuning pretrained models with Bayesian methods makes it possible to use these large models for uncertainty quantification \citep{krishnan2020moped,den2023bayes-adapter}.
As typically only a single pretrained model is available, we initialize all ensemble members from the same model, with only the classification head being initialized randomly.
For BBB, Rank-1 VI, and iVON, we only make the randomly initialized classification head Bayesian.
This reduces the computational overhead significantly and sidesteps the cold posterior effect \citep{wenzel2020tempering} of BBB, as our experiments show.
The concept is similar to the last-layer models used by \citet{foong2019gap} and \citet{ovadia2019ood-comparison}.
For a fair comparison we also experimented with last-layer versions of MCD, SVGD, and SWAG, but found generalization capability and calibration to decrease.
See the individual sections below for details.



\begin{figure}[!t]
    \centering
    \begin{subfigure}[t]{.4\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{paretoplot}{data/iwildcam.dat}{macro f1}{macro f1_std}{sece}{sece_std}{
                    paretostyle,
                    xlabel=Macro F1 Score,
                    ylabel=sECE,
                    width=10cm,
                    yticklabel style={
                        /pgf/number format/fixed,
                        /pgf/number format/precision=2
                    }
                }
                
                \modelparetoplot{map-1}{MAP}{color=map, single}
        
                \modelparetoplot{mcd_p0.1-1}{MCD}{color=mcd, single}
        
                \modelparetoplot{swag-1}{SWAG}{color=swag, single}
        
                \modelparetoplot{laplace-1}{Laplace}{color=laplace, single}
                
                \modelparetoplot{bbb-1}{BBB}{color=bbb, single}
                
                \modelparetoplot{rank1-1}{Rank-1 VI}{color=rank1, single}
                
                \modelparetoplot{map_5}{Deep Ensemble}{color=map, multix}
        
                \modelparetoplot{mcd_5}{MultiMCD}{color=mcd, multix}
        
                \modelparetoplot{swag_5}{MultiSWAG}{color=swag, multix}
        
                \modelparetoplot{bbb_5}{MultiBBB}{color=bbb, multix}
        
                \modelparetoplot{laplace_5}{MultiLaplace}{color=laplace, multix}
                
                \modelparetoplot{svgd-1}{SVGD}{color=svgd, single}

                \modelparetoplot{ll_ivon-1}{iVON}{color=ivon, single}
                \modelparetoplot{ll_ivon_5}{MultiiVON}{color=ivon, multix}
            \end{paretoplot}
        }
        \caption{\dataset{iWildCam-wilds}}
        \label{fig:iwildcam}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.4\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{paretoplot}{data/fmow.dat}{worst_acc accuracy}{worst_acc accuracy_std}{worst_acc sece}{worst_acc sece_std}{
                    paretostyle,
                    xlabel=Accuracy (Worst Region),
                    ylabel=sECE (Worst Region),
                    width=10cm,
                    legend columns = 4,
                    legend style = {
                        at = {(0.5, -0.2)},
                        anchor=north
                    },
                    yticklabel style={
                        /pgf/number format/fixed,
                        /pgf/number format/precision=2
                    }
                }
                
                \modelparetoplot{map-1}{MAP}{color=map, single}
        
                \modelparetoplot{mcd_p0.1-1}{MCD}{color=mcd, single}
        
                \modelparetoplot{swag-1}{SWAG}{color=swag, single}
                
                \modelparetoplot{bbb-1}{BBB}{color=bbb, single}

                \modelparetoplot{rank1-1}{Rank-1 VI}{color=rank1, single}
                
                \modelparetoplot{map-5}{MAP}{color=map, multix}
        
                \modelparetoplot{mcd-5}{MCD}{color=mcd, multix}
        
                \modelparetoplot{swag-5}{SWAG}{color=swag, multix}
        
                \modelparetoplot{bbb-5}{BBB}{color=bbb, multix}
        
                \modelparetoplot{svgd-1}{SVGD}{color=svgd, single}

                \modelparetoplot{ll_ivon-1}{iVON}{color=ivon, single}
                \modelparetoplot{ll_ivon-5}{MultiiVON}{color=ivon, multix}
            \end{paretoplot}
        }
        \caption{\dataset{FMoW-wilds}}
        \label{fig:fmow}
    \end{subfigure}
    \begin{subfigure}[b]{.15\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{tikzpicture}
                \begin{axis}[
                        paretostyle, 
                        hide axis, 
                        xmin=0, xmax=1, ymin=0, ymax=1,
                        legend columns = 1,
                        legend style = {
                            legend cell align=left
                        }
                    ]
                    \addlegendimage{color=map, single}
                    \addlegendentry{MAP};
                    
                    \addlegendimage{color=map, multix}
                    \addlegendentry{Deep Ensemble};
            
                    \addlegendimage{color=mcd, single}
                    \addlegendentry{MCD};
            
                    \addlegendimage{color=mcd, multix}
                    \addlegendentry{MultiMCD};
            
                    \addlegendimage{color=swag, single}
                    \addlegendentry{SWAG};
            
                    \addlegendimage{color=swag, multix}
                    \addlegendentry{MultiSWAG};
                    
                    \addlegendimage{color=bbb, single}
                    \addlegendentry{BBB};
            
                    \addlegendimage{color=bbb, multix}
                    \addlegendentry{MultiBBB};
            
                    \addlegendimage{color=laplace, single}
                    \addlegendentry{Laplace};
            
                    \addlegendimage{color=laplace, multix}
                    \addlegendentry{MultiLaplace};
                    
                    \addlegendimage{color=rank1, single}
                    \addlegendentry{Rank-1 VI};
                    
                    \addlegendimage{color=ivon, single}
                    \addlegendentry{iVON};
                    
                    \addlegendimage{color=ivon, multix}
                    \addlegendentry{MultiiVON};
                    
                    \addlegendimage{color=svgd, single}
                    \addlegendentry{SVGD};
                \end{axis}
            \end{tikzpicture}
        }
        \vspace{0.2cm}
        \vskip 0pt
    \end{subfigure}
    \caption{Macro F1 Score / Worst-Region Accuracy vs. sECE on the o.o.d. evaluation splits of the image classification finetuning tasks \dataset{iWildCam-wilds} and \dataset{FMoW-wilds}. Among the single-mode approximations, BBB is better calibrated but less accurate than SWAG and MCD. iVONs calibration is inconsistent: On \dataset{iWildCam} it is better calibrated than BBB, but on \dataset{FMoW} it barely performs better than MAP. Laplace is very well calibrated on \dataset{iWildCam}, but underperforms on \dataset{FMoW} and is therefore excluded on this dataset. All MultiX algorithms and the Deep Ensemble are more accurate and better calibrated than any single-mode approximation. SVGD performs very similar to MAP in regard to both metrics, even though it uses a multi-mode posterior approximation.}
    \label{fig:iwildcam-fmow}
\end{figure}

\subsubsection{Finetuning Convolutional Neural Networks}
\label{sec:image-classification}
For all tasks we use the pretrained parameter checkpoints provided by PyTorch \citep{gardner2018gpytorch}.
As ResNets and DenseNets typically do not include dropout, we only add a single dropout layer directly before the freshly initialized linear classification layer.
We do not use running statistics for the batch normalization layers during evaluation.
This eliminates any bias on the o.o.d. datasets that batch normalization might introduce, and alleviates the need to re-initialize the normalization layers after sampling model parameters. 
See \Cref{sec:batchnorm} for a more detailed discussion.

\paragraph{Tasks}
\textbf{\dataset{iWildCam-wilds}} \citep{beery2020iwildcam} is an image classification task that consists of animal photos taken by camera traps across the world.
The model's task is to determine which of 182 animal species can be seen in the image.
As rare animal species, which are of special interest to researchers, are naturally underrepresented in the dataset, the F1 score is used to evaluate the predictive performance.
The o.o.d. evaluation split consists of images from new camera locations.
See \Cref{sec:iwildcam-details} for details.
\textbf{\dataset{FMoW-wilds}} (Functional Map of the World) \citep{christie2018fmow} is an image classification task, where the inputs are satellite images and the classes are building and land use categories.
The o.o.d. evaluation split consists of images from different years than the images in the training set.
Models are separately evaluated on five geographical regions of the world, with the lowest accuracy taken as the main evaluation metric.
\Cref{fig:fmow} shows the results for most algorithms.
See \Cref{sec:fmow-details} for details.
\textbf{\dataset{RxRx1-wilds}} \citep{taylor2019rxrx1} is an image classification task, where the inputs are three-channel images of cells, and the classes are 1139 applied genetic treatments.
In high-throughput medical and biological screening applications, experiments are typically batched together.
This leads to multiple experiments being affected by similar confounding factors, making it hard to draw conclusions between different batches.
Batches that were unseen during training form the o.o.d. evaluation split of \dataset{RxRx1}.
As noted by \citet{koh2021wilds} the task is very hard given that only three of the six available input channels are used which leads to the low accuracy of most models.
See \Cref{sec:rxrx1-details} for details.

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{tikzpicture}
                \begin{groupplot}[
                        paretostyle,
                        group style = {
                            group size = 1 by 2,
                            xticklabels at=edge bottom,
                            vertical sep = 0pt
                        },
                        legend columns = 1,
                        legend style = {
                            at = {(1.1, -0.5)},
                            anchor=west,
                            font=\footnotesize,
                            legend cell align=left
                        },
                        legend image post style={scale=0.7},
                        xticklabel style={
                            /pgf/number format/fixed,
                            /pgf/number format/precision=3
                        },
                        width=8cm,
                        xmin=0.07, xmax=0.13,
                    ]
                    \newcommand{\bayesdatafile}{data/rxrx1.dat}
                    \newcommand{\bayesxcol}{ood accuracy}
                    \newcommand{\bayesxerr}{ood accuracy_std}
                    \newcommand{\bayesycol}{ood sece}
                    \newcommand{\bayesyerr}{ood sece_std}
                    \newcommand{\bayesmodelcol}{model}
            
                    \nextgroupplot[axis x line=top, axis y discontinuity=parallel, ymin=-0.1399, ymax=0.0, height=3.8889cm]
                        \modelparetoplot{map_1}{MAP}{color=map, single}
                        \addlegendentry{MAP}
                        \modelparetoplot{mcd_1}{MCD}{color=mcd, single}
                        \addlegendentry{MCD}
                        \modelparetoplot{swag_1}{SWAG}{color=swag, single}
                        \addlegendentry{SWAG}
                        \modelparetoplot{svgd_1}{SVGD}{color=svgd, single}
                        \addlegendentry{SVGD}
                        
                        \modelparetoplot{map_5}{MAP}{color=map, multix}
                        \addlegendentry{Deep Ensemble}
                        \modelparetoplot{mcd_5}{MCD}{color=mcd, multix}
                        \addlegendentry{MultiMCD}
                        \modelparetoplot{swag_5}{SWAG}{color=swag, multix}
                        \addlegendentry{MultiSWAG}
            
                    \nextgroupplot[axis x line=bottom, ymin=-0.42, ymax=-0.24, height=5cm, xlabel=Accuracy, ylabel=sECE]
                        \modelparetoplot{map_1}{MAP}{color=map, single}
                        \modelparetoplot{mcd_1}{MCD}{color=mcd, single}
                        \modelparetoplot{swag_1}{SWAG}{color=swag, single}
                        \modelparetoplot{svgd_1}{SVGD}{color=svgd, single}
                        
                        \modelparetoplot{map_5}{MAP}{color=map, multix}
                        \modelparetoplot{mcd_5}{MCD}{color=mcd, multix}
                        \modelparetoplot{swag_5}{SWAG}{color=swag, multix}
                \end{groupplot}
            \end{tikzpicture}
        }
        \caption{Non-VI Algorithms and SVGD}
        \label{fig:rxrx1-non-vi}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.5\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{paretoplot}{data/rxrx1.dat}{ood accuracy}{ood accuracy_std}{ood sece}{ood sece_std}{
                    paretostyle,
                    xlabel=Accuracy,
                    ylabel=sECE,
                    width=10cm,
                    legend columns = 1,
                    legend style = {
                        at = {(1.05, 0.5)},
                        anchor=west,
                        legend cell align=left
                    },
                    xticklabel style={
                        /pgf/number format/fixed,
                        /pgf/number format/precision=3
                    }
                }
                \modelparetoplot{bbb_1}{BBB}{color=bbb, single}
                \addlegendentry{BBB ($\sigma=1.0, \lambda=1.0$)};
                \modelparetoplot{bbb_prior0.1_1}{BBB}{color=swag, single}
                \addlegendentry{BBB ($\sigma=0.1, \lambda=1.0$)};
                \modelparetoplot{bbb_prior0.5_1}{BBB}{color=laplace, single}
                \addlegendentry{BBB ($\sigma=0.5, \lambda=1.0$)};
                \modelparetoplot{bbb_kl0.2_1}{BBB}{color=mcd, single}
                \addlegendentry{BBB ($\sigma=1.0, \lambda=0.2$)};
                \modelparetoplot{rank1_1}{Rank-1 VI}{color=rank1, single}
                \modelparetoplot{ll_ivon_1}{iVON}{color=ivon, single}
                \addlegendentry{Rank-1 VI};
            \end{paretoplot}
        }
        \caption{BBB and Rank-1 VI}
        \label{fig:rxrx1-vi}
    \end{subfigure}
    
    \caption{\dataset{RxRx1-wilds}: Accuracy vs. sECE on the o.o.d. evaluation split. Ensembles are more accurate and significantly better calibrated than all single-mode approximations (\Cref{fig:rxrx1-non-vi}, note the split y-axis). SVGD performs similar to MAP, even though it is based on an ensemble.
We also experimented with a last-layer version of SVGD on \dataset{iWildCam}, but found only a small increase in the macro F1 score. (\Cref{sec:iwildcam-details}). MAP is the best calibrated non-VI single-mode approximation. The VI algorithms except for SVGD are significantly less accurate than all other models. BBB becomes slightly more accurate with colder posterior temperatures $\lambda$, but less accurate with smaller prior standard deviations $\sigma$ (\Cref{fig:rxrx1-vi}). Laplace also underperforms and is therefore excluded.}
    \label{fig:rxrx1}
\end{figure}


\paragraph{Generalization}
MultiX algorithms generalize better than the corresponding single-mode algorithms, with MultiSWAG and MultiMCD performing particularly well.
The relative ordering of the MultiX models depends on the dataset and does not always correlate with the relative ordering of the corresponding single-mode approximations: For example is MCD slightly less accurate than MAP on \dataset{FMoW}, but MultiMCD is significantly more accurate than the Deep Ensemble.
On \dataset{iWildCam}, the single-mode posterior approximations SWAG and MCD are competitive with the Deep Ensemble.
SVGD performs similar to MAP, even though it is based on an ensemble, likely due to the repulsive forces pushing the particles away from the well-performing pretrained model.
We also experimented with a last-layer version of SVGD on \dataset{iWildCam}, but found only a small increase in the macro F1 score. (\Cref{sec:iwildcam-details}).
While the VI algorithms' accuracy is similar to the accuracy of MAP on \dataset{iWildCam} and \dataset{FMoW}, all VI algorithms except SVGD perform significantly worse than the non-VI algorithms on \dataset{RxRx1}.
We experimented with different prior standard deviations $\sigma$ and scaling factors $\lambda$ for the KL divergence in \Cref{fig:rxrx1-vi} and found only a small accuracy increase.
Similarly, Laplace underfits on \dataset{FMoW} and \dataset{RxRx1} (see \Cref{sec:fmow-details} and \Cref{sec:rxrx1-details}).

\paragraph{Calibration}
MultiX algorithms are consistently better calibrated than any single-mode algorithm, with a tendency of becoming underconfident on \dataset{iWildCam}.
Again, we find that MultiX generally performs better than a Deep Ensemble.
However, MultiSWAG in particular is more overconfident than the Deep Ensemble, even though SWAG is better calibrated than MAP.
BBB is better calibrated than other single-mode approximations such as SWAG and MCD.
On \dataset{iWildCam}, Laplace is the best calibrated single-mode approximation, and correspondingly MultiLaplace is the most underconfident multi-mode approximation.
This result is unique to \dataset{iWildCam}, as Laplace underfits on the other image classification datasets.


\FloatBarrier
\subsubsection{Finetuning Transformers}
\label{sec:text-classification}
Transformers-based models are underrepresented in the literature on Bayesian deep learning, despite their recent success in deep learning in general \citep{brown2020gpt3}.
We use the \dataset{CivilComments-wilds} and \dataset{Amazon-wilds} datasets to evaluate the Bayesian algorithms on the transformer-based DistilBERT \citep{sanh2019distilbert} architecture.
Similar to the computer vision tasks, we initialize all models from the same pretrained model checkpoint.

\paragraph{Tasks}
\textbf{\dataset{CivilComments-wilds}} \citep{borkan2019civilcomments} is a binary text classification dataset, where the model's task is to classify whether a given comment is toxic or not.
The comments are grouped based on whether they mention certain demographic groups, such as LGBTQ or muslim identities.
Models are evaluated based on the group on which they achieve the lowest accuracy on the evaluation set.
See \Cref{sec:civil-details} for details.
\textbf{\dataset{Amazon-wilds}} \citep{ni2019amazon} consists of textual product reviews where the task is to predict the star rating from one to five.
The o.o.d. evaluation split consists of reviews from reviewers that are not part of the training split.
Models are evaluated based on the accuracy of the review at the $10\%$ quantile.
See \Cref{sec:amazon-details} for details.

\begin{figure}[!t]
    \centering
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{paretoplot}{data/civil.dat}{worst_acc accuracy}{worst_acc accuracy_std}{worst_acc sece}{worst_acc sece_std}{
                    paretostyle,
                    xlabel=Accuracy (Worst Group),
                    ylabel=sECE (Worst Group),
                    height=10cm, width=10cm
                }
                
                \modelparetoplot{map}{MAP}{color=map, single}
                \modelparetoplot{map_4}{Deep Ensemble}{color=map, multix}
        
                \modelparetoplot{mcd}{MCD}{color=mcd, single}
                \modelparetoplot{mcd_4}{MultiMCD}{color=mcd, multix}
        
                \modelparetoplot{swag}{SWAG}{color=swag, single}
                \modelparetoplot{swag_4}{MultiSWAG}{color=swag, multix}
            
                \modelparetoplot{laplace}{Laplace}{color=laplace, single}
                \modelparetoplot{laplace_4}{MultiLaplace}{color=laplace, multix}
        
                \modelparetoplot{bbb}{BBB}{color=bbb, single}
                \modelparetoplot{bbb_4}{MultiBBB}{color=bbb, multix}
                
                \modelparetoplot{rank1}{Rank-1 VI}{color=rank1, single}
                \modelparetoplot{ll_ivon}{iVON}{color=ivon, single}
                \modelparetoplot{ll_ivon_5}{MultiiVON}{color=ivon, multix}
                \modelparetoplot{svgd}{SVGD}{color=svgd, single}
            \end{paretoplot}
        }
        \caption{\dataset{CivilComments-wilds}}
        \label{fig:civil}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{paretoplot}{data/amazon.dat}{ood 10th_percentile_acc}{ood 10th_percentile_acc_std}{ood sece}{ood sece_std}{
                    paretostyle,
                    xlabel=$10\%$ Accuracy,
                    ylabel=sECE,
                    height=10cm, width=10cm
                }
                
                \modelparetoplot{map}{MAP}{color=map, single}
                \modelparetoplot{map_5}{Deep Ensemble}{color=map, multix}
        
                \modelparetoplot{mcd}{MCD}{color=mcd, single}
                \modelparetoplot{mcd_5}{MultiMCD}{color=mcd, multix}
        
                \modelparetoplot{swag}{SWAG}{color=swag, single}
                \modelparetoplot{swag_5}{MultiSWAG}{color=swag, multix}
        
                \modelparetoplot{bbb}{BBB}{color=bbb, single}
                \modelparetoplot{bbb_5}{MultiBBB}{color=bbb, multix}
                \modelparetoplot{rank1}{Rank-1 VI}{color=rank1, single}
                \modelparetoplot{ll_ivon}{iVON}{color=ivon, single}
                \modelparetoplot{ll_ivon_5}{MultiiVON}{color=ivon, multix}
                \modelparetoplot{laplace_1}{Laplace}{color=laplace, single}
                \modelparetoplot{laplace_5}{MultiLaplace}{color=laplace, multix}
                \modelparetoplot{svgd}{SVGD}{color=svgd, single}
            \end{paretoplot}
        }
        \caption{\dataset{Amazon-wilds}}
        \label{fig:amazon}
    \end{subfigure}
    \begin{subfigure}[b]{0.13\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \begin{tikzpicture}
                \begin{axis}[
                        paretostyle,
                        xmin=0, xmax=1, ymin=0, ymax=1,
                        hide axis,
                        legend columns=1,
                        legend style={
                            legend cell align=left
                        }
                    ]
                    
                    \addlegendimage{color=map, single}
                    \addlegendentry{MAP};
                    \addlegendimage{color=map, multix}
                    \addlegendentry{Deep Ensemble};
            
                    \addlegendimage{color=mcd, single}
                    \addlegendentry{MCD};
                    \addlegendimage{color=mcd, multix}
                    \addlegendentry{MultiMCD};
            
                    \addlegendimage{color=swag, single}
                    \addlegendentry{SWAG};
                    \addlegendimage{color=swag, multix}
                    \addlegendentry{MultiSWAG};
                    
                    \addlegendimage{color=laplace, single}
                    \addlegendentry{Laplace};
                    \addlegendimage{color=laplace, multix}
                    \addlegendentry{MultiLaplace};
            
                    \addlegendimage{color=bbb, single}
                    \addlegendentry{BBB};
                    \addlegendimage{color=rank1, single}
                    \addlegendentry{Rank-1 VI};
                    \addlegendimage{color=ivon, single}
                    \addlegendentry{iVON};
                    \addlegendimage{color=ivon, multix}
                    \addlegendentry{MultiiVON};
                    \addlegendimage{color=svgd, single}
                    \addlegendentry{SVGD};
                \end{axis}
            \end{tikzpicture}
        }
        \vspace{0.8cm}
        \vskip 0pt
    \end{subfigure}
    \hfill\phantom{i}
    \caption{Text classification with pretrained transformers. With the exception of MultiBBB on \dataset{Amazon-wilds}, ensembles perform nearly identical to the corresponding single-mode approximations. VI improves the accuracy of the models.}
    \label{fig:civil-amazon}
\end{figure}



\paragraph{Generalization}
On both tasks BBB and Rank-1 VI are the most accurate models, with no benefit from the multiple components of Rank-1 VI.
Interestingly, iVON is significantly less accurate than BBB, even though it is also based on mean-field variational inference.
Therefore the natural gradients seem to be disadvantageous on the transformer-based architecture that we use.
To see whether the better performance of BBB is due to less regularization compared to MAP, we also experimented with a smaller weight decay factor for MAP on \dataset{CivilComments}.
While we found that the accuracy increased, BBB was still more accurate (see \Cref{sec:civil-details}).
Finally, we also checked whether the better performance of BBB is due to its last-layer nature.
We experimented with last-layer versions of MCD and SWAG on \dataset{Amazon} (see \Cref{sec:amazon-details}), but found that both were still significantly less accurate than BBB.

Ensemble-based models are no more accurate than the corresponding single-mode approximations, contrary to the results on all other datasets.
We suspect that this effect is to a large part due to the finetuning nature of the tasks, where all ensemble members start close to each other in parameter space and therefore converge to the same posterior mode.
Note that the failure of ensembles is most likely due to the task and the network architecture, and not due to the training procedure: While we train for fewer epochs than on the image classification tasks, the datasets are larger.
On \dataset{iWildCam} we perform 97k parameter updates and on \dataset{RxRx1} 48k parameter updates during training, compared to 84k parameter updates on \dataset{CivilComments}.

MCD is the least accurate model on \dataset{CivilComments}.
We experimented with different dropout rates in \Cref{sec:civil-details} and found that MCD performs better with smaller dropout rates, but becomes never more accurate than MAP.

\paragraph{Calibration}
SWAG is the least confident model on both tasks, which leads to underconfidence on \dataset{Amazon}.
MCD's calibration is inconclusive: While it is better calibrated than MAP on \dataset{Amazon}, it is more overconfident on \dataset{CivilComments}.
With the exception of MultiBBB on \dataset{Amazon}, ensembles are not better calibrated than the respective single-mode approximations.
BBB and Rank-1 VI are not better calibrated than MAP and on \dataset{Amazon} significantly more overconfident than \dataset{MAP}.


